Scaling LLaNA: Advancing NeRF-Language Understanding Through Large-Scale Training

Recent advances in Multimodal Large Language Models (MLLMs) have shown remarkable capabilities in understanding both images and 3D data, yet these modalities face inherent limitations in comprehensively representing object geometry and appearance. Neural Radiance Fields (NeRFs) have emerged as a promising alternative, encoding both geometric and photorealistic properties within the weights of a simple Multi-Layer Perceptron (MLP). This work investigates the feasibility and effectiveness of ingesting NeRFs into an MLLM. We introduce LLaNA, the first MLLM able to perform new tasks such as NeRF captioning and Q\&A, by directly processing the weights of a NeRF's MLP. Notably, LLaNA is able to extract information about the represented objects without the need to render images or materialize 3D data structures. In addition, we build the first large-scale NeRF-language dataset, composed by more than 300K NeRFs trained on ShapeNet and Objaverse, with paired textual annotations that enable various NeRF-language tasks. Based on this dataset, we develop a benchmark to evaluate the NeRF understanding capability of our method. Results show that directly processing NeRF weights leads to better performance on NeRF-Language tasks compared to approaches that rely on either 2D or 3D representations derived from NeRFs.

==> sections/extra.tex <==
%\clearpage
\begin{figure*}[t!]
    \centering
    \caption{\textbf{ObjaNeRF-Text statistics for ground-truth brief and detailed descriptions.}}

    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c}
    \begin{tabular}{cccc}
    \multicolumn{2}{c}{\small Brief Descriptions - Word clouds} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/brief_description instruction.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/brief_description response.pdf} \\
    {\small Instructions} & {\small Responses} \\
    
    \multicolumn{2}{c}{\small Brief Descriptions - Lengths (Words)} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/brief_description instruction_lengths.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/brief_description response_lengths.pdf} \\
    {\small Instructions} & {\small Responses} \\

    \multicolumn{2}{c}{\small Detailed Descriptions - Word clouds} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/detailed_description instruction.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/detailed_description response.pdf} \\
    {\small Instructions} & {\small Responses} \\
    
    \multicolumn{2}{c}{\small Detailed Descriptions - Lengths (Words)} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/detailed_description instruction_lengths.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/detailed_description response_lengths.pdf} \\
    {\small Instructions} & {\small Responses} \\

    \end{tabular} 
    \end{tabular}
    \label{tab:dataset_stats_cap}
\end{figure*}
\clearpage

\clearpage
\begin{figure*}[t!]
    \centering
    \caption{\textbf{ObjaNeRF-Text statistics for ground-truth single-round and multi-round Q\&A.}}

    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c}
    \begin{tabular}{cc}
    \multicolumn{2}{c}{\small Single-round Q\&A - Word clouds} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/single_round_instruction.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/single_round_response.pdf} \\
    {\small Instructions} & {\small Responses} \\
    
    \multicolumn{2}{c}{\small Single-round Q\&A - Lengths (Words)} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/single_round_instruction_lengths.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/single_round_response_lengths.pdf} \\
    {\small Instructions} & {\small Responses} \\

    \multicolumn{2}{c}{\small Multi-round Q\&A - Word clouds} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/multi_round_instruction.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/multi_round_response.pdf} \\
    {\small Instructions} & {\small Responses} \\
    
    \multicolumn{2}{c}{\small Multi-round Q\&A - Lengths (Words)} \\
    \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/multi_round_instruction_lengths.pdf} & \includegraphics[width=0.5\linewidth]{figures/objanerf_text_stats/train/multi_round_response_lengths.pdf} \\
    {\small Instructions} & {\small Responses} \\

    \end{tabular} 
    \end{tabular}
    \label{tab:dataset_stats_qa}
\end{figure*}
\clearpage

==> tables/language_only_baselines_classification.tex <==
\begin{table}[t!]
    \centering
    \caption{\textbf{Language-only baselines on zero-shot NeRF classification}}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{lllccccc}
        \midrule
        \textbf{Model} & \textbf{Accuracy (\%)} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2}
        LLaMA-7b  & 6.27 \\
        LLaMA-13b & 2.36 \\
        \bottomrule
        \end{tabular}}
        \label{tab:language_only_classification}
\end{table}

==> tables/shapenerf_trained_brief.tex <==
%%% Brief descriptions dataset
\begin{table}[t]
    \centering
    \caption{\textbf{NeRF brief captioning on ShapeNeRF--Text.} All methods trained on ShapeNeRF--Text training set. Best results are in \textbf{bold}, runner-up is \underline{underlined}. \\(FV: front-view, MV: multi-view)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccccc}
        \midrule
        \textbf{Model} & \textbf{Modality} & \textbf{S-BERT} & \textbf{SimCSE} & \textbf{BLEU-1} & \textbf{ROUGE-L} & 
        \textbf{METEOR} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        GPT4Point-Opt-2.7b & Point cloud & 37.96 & 39.00 & 21.33 & 22.29 & \underline{24.88} \\
        PointLLM-7b & Point cloud & \underline{55.48} & \underline{57.28} & \underline{21.67} &   \underline{25.84} & 24.54 \\
        %\model{}-7b & \nerf{} & 68.63 & 70.54 & 20.64 & 28.33 & 31.76 \\
        \model{}-7b & \nerf{} & \textbf{76.04} & \textbf{77.13} & 
        \textbf{45.00} & \textbf{45.87} & \textbf{44.52} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        \llava{}-vicuna-13b & Image (FV) & 42.86 & 43.22 & 15.56 & 13.74 & 15.27 \\
        \llava{}-vicuna-13b & Image (MV) & 44.29 & 41.85 & 16.67 & 16.26 & 17.58 \\
        \bottomrule
        \end{tabular}}
    \label{tab:brief_trained}
\end{table}

==> tables/shapenerf_trained_detailed.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{NeRF detailed captioning on ShapeNeRF--Text.} All methods trained on ShapeNeRF--Text training set. Best results are in \textbf{bold}, runner-up is \underline{underlined}. \\(FV: front-view, MV: multi-view)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccccc}
        \midrule
        \textbf{Model} & \textbf{Modality} & \textbf{S-BERT} & \textbf{SimCSE} & \textbf{BLEU-1} & \textbf{ROUGE-L} & \textbf{METEOR} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        GPT4Point-Opt-2.7b & Point cloud & 41.33 & 40.52 & 14.48 & 19.15 & \underline{13.80} \\
        PointLLM-7b & Point cloud & \underline{67.30} & \underline{59.56} & \underline{15.39} & 21.42 & 11.37 \\
        %\model{}-7b & \nerf{} & \textbf{77.43} & \textbf{79.81} & \textbf{41.32} & \textbf{36.18} & \textbf{32.39} \\
        \model{}-7b & \nerf{} & \textbf{75.83} & \textbf{77.92} & \textbf{20.22} & \textbf{33.80} & \textbf{21.20} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        \llava{}-vicuna-13b & Image (FV) & 44.69 & 42.31 & 10.08 & 23.46 & 12.70 \\   
        \llava{}-vicuna-13b & Image (MV) & 45.72 & 42.49 & 12.17 & \underline{23.48} & 14.25 \\
        \bottomrule
        \end{tabular}}
    \label{tab:detailed_trained}
\end{table}

==> tables/shapenerf_trained_hst.tex <==
%%% HST dataset
\begin{table}[t]
    \caption{\textbf{NeRF brief captioning on the HST dataset.} All methods trained on ShapeNeRF--Text training set. Best results are in \textbf{bold}, runner-up is \underline{underlined}. \\(FV: front-view, MV: multi-view)}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccccc}
        \midrule
        \textbf{Model} & \textbf{Modality} & \textbf{S-BERT} & \textbf{SimCSE} & \textbf{BLEU-1} & \textbf{ROUGE-L} & \textbf{METEOR} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        GPT4Point-Opt-2.7B & Point cloud & 30.50 & 31.08 & 8.12 & 12.35 & 11.62 \\
        PointLLM-7b & Point cloud & \underline{44.65} & \underline{44.68} & 8.91 & 12.33 &  \underline{12.64} \\
        %\model{}-7b & \nerf{} & \underline{55.62} & \underline{55.56} & 6.56 & 11.81 & \underline{14.52}  \\
        \model{}-7b & \nerf{} & \textbf{65.42} & \textbf{66.44} & \textbf{19.63} & \textbf{23.39} & \textbf{23.46} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        \llava{}-vicuna-13b & Image (FV) & 33.79 & 42.66 & 10.28 & \underline{13.22} & 12.19 \\   
        \llava{}-vicuna-13b & Image (MV) & 34.45 & 42.54 & \underline{11.04} & 12.36 & 11.48 \\ 
        \bottomrule
        \end{tabular}}
    \label{tab:brief_trained_hst}
\end{table}

==> tables/shapenerf_trained_qa.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{NeRF single-round Q\&A on ShapeNeRF--Text.} All methods trained on ShapeNeRF--Text training set. Best results are in \textbf{bold}, runner-up is \underline{underlined}. \\(FV: front-view, MV: multi-view)}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{lcccccc}
        \midrule
        \textbf{Model} & \textbf{Modality} & \textbf{S-BERT} & \textbf{SimCSE} & \textbf{BLEU-1} & \textbf{ROUGE-L} & \textbf{METEOR} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        GPT4Point-Opt-2.7b & Point cloud & 22.22 & 28.66 & 8.76 & 13.46 & 14.19 \\
        PointLLM-7b & Point cloud & \underline{79.24} & \underline{80.38} & \underline{46.00} & \underline{52.60} & \underline{42.36} \\
        %\model{}-7b & \nerf{} & \underline{81.03} & \underline{81.56} & \underline{46.16} & \underline{53.17} & \underline{50.15} \\
        \model{}-7b & \nerf{} & \textbf{81.94} & \textbf{82.43} & \textbf{47.73} & \textbf{54.97} & \textbf{51.78} \\
        \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-7}
        \llava{}-vicuna-13b & Image (FV) & 56.29 & 62.36 & 26.87 & 29.55 & 30.49 \\    
        \llava{}-vicuna-13b & Image (MV) & 56.42 & 64.47 & 25.41 & 30.09 & 32.04 \\     
        \bottomrule
        \end{tabular}}
    \label{tab:qa_trained}
\end{table}
